Efficient Approximate Kernel Based Spike Sequence Classification

Machine learning (ML) models, such as SVM, for tasks like classification and clustering of sequences, require a definition of distance/similarity between pairs of sequences. Several methods have been proposed to compute the similarity between sequences, such as the exact approach that counts the number of matches between $k$-mers (sub-sequences of length $k$) and an approximate approach that estimates pairwise similarity scores. Although exact methods yield better classification performance, they pose high computational costs, limiting their applicability to a small number of sequences. The approximate algorithms are proven to be more scalable and perform comparably to (sometimes better than) the exact methods -- they are designed in a "general" way to deal with different types of sequences (e.g., music, protein, etc.). Although general applicability is a desired property of an algorithm, it is not the case in all scenarios. For example, in the current COVID-19 (coronavirus) pandemic, there is a need for an approach that can deal specifically with the coronavirus. To this end, we propose a series of ways to improve the performance of the approximate kernel (using minimizers and information gain) in order to enhance its predictive performance pm coronavirus sequences. More specifically, we improve the quality of the approximate kernel using domain knowledge (computed using information gain) and efficient preprocessing (using minimizers computation) to classify coronavirus spike protein sequences corresponding to different variants (e.g., Alpha, Beta, Gamma). We report results using different classification and clustering algorithms and evaluate their performance using multiple evaluation metrics. Using two datasets, we show that our proposed method helps improve the kernel's performance compared to the baseline and state-of-the-art approaches in the healthcare domain.

==> Makefile <==
targets = main.pdf abstract.txt
figs =

all : $(targets)

# custom main
main.pdf : main.tex kernel_Computation_Detail.tex figures bibliography.bib
	latexmk -pdf $< && latexmk -c $<

# abstract
abstract.txt : main.tex
	grep -A 1000 "begin{abstract}" $< \
		| tail -n +2 \
		| grep -B 1000 "end{abstract}" \
		| head -n -1 > $@

# figures
.PHONY : figures
figures : $(figs)
	for fig in $^ ; do \
		cd $$fig && make && cd .. ; \
	done

# cleanup
.PHONY : clean scour
clean :
	rm -f *~
	rm -f *.aux *.bbl *.log *.out

scour : clean
	rm -f $(targets)

